Context-Dependent Implicit Authentication for Wearable Device User

As market wearables are becoming popular with a range of services, including making financial transactions, accessing cars, etc. that they provide based on various private information of a user, security of this information is becoming very important. However, users are often flooded with PINs and passwords in this internet of things (IoT) world. Additionally, hard-biometric, such as facial or finger recognition, based authentications are not adaptable for market wearables due to their limited sensing and computation capabilities. Therefore, it is a time demand to develop a burden-free implicit authentication mechanism for wearables using the less-informative soft-biometric data that are easily obtainable from the market wearables. In this work, we present a context-dependent soft-biometric-based wearable authentication system utilizing the heart rate, gait, and breathing audio signals. From our detailed analysis, we find that a binary support vector machine (SVM) with radial basis function (RBF) kernel can achieve an average accuracy of $0.94 \pm 0.07$, $F_1$ score of $0.93 \pm 0.08$, an equal error rate (EER) of about $0.06$ at a lower confidence threshold of 0.52, which shows the promise of this work.

==> introduction.tex <==
\section{Introduction}\label{introduction}

\subsection{Motivation}
Internet of Things (IoT) has increased our access to a multitude of devices with advanced capabilities that allow us to remotely collect information or control physical objects.
\ignore{Various examples of such systems include alarm systems, entertainment devices, vehicles, and smart home devices, to name a few. IoT systems are connected to existing network infrastructure providing new interfaces that integrate the physical world with computer-based systems.} 
Along with the growth of IoT, smartphones and wearables have advanced in their sensing and computational capabilities to a point which enable many new applications and usage scenarios to emerge.\ignore{ While smartphones are already widely used \cite{seneviratne2017survey},} On the other hand, wearables are relatively new and still growing in popularity with the arrival of new applications. Some include the ability to identify a user to third party services \cite{bianchi2016wearable}, store sensitive user information (i.e., passwords, credit card information) \cite{nguyen2017smartwatches}, manage financial payments \cite{seneviratne2017survey}, access phones and other paired devices \cite{kumar2016authenticating}, unlock vehicles \cite{nguyen2017smartwatches}, monitor or track individuals (e.g., child monitoring or fall detection), and assess an individual's health and fitness. According to a recent market report, a 72.7\% increase in wearable shipments and an associated increase in sales revenue of 78.1\% are predicted from 2016 to 2022~\cite{wearable_shipments_revenue}. 

However, wearables also raise new challenges, especially in terms of security. Unauthorized access to a wearable can enable imposters to steal information from other sensitive IoT objects, which poses a significant risk \cite{zeng2017wearia}.\ignore{Unauthorized users could also steal data on the wearables itself, e.g., many applications and services provided by a wearable depend on sensor and user data stored on the device to grant access.} Another concern is the reliability and accuracy of the physiological and activity data collected by wearables. Many healthcare providers and researchers rely on wearables to monitor their patients or study participants remotely and an intentional device sharing between target and non-target users might lead to inaccurate and faulty assessment. Therefore, there is an imperative need for a robust and accurate authentication mechanism specifically for wearable device users.

Existing wearable devices either have no authentication systems or authentication mechanisms that are often knowledge-based regular PIN locks or pattern locks \cite{nguyen2017smartwatches}, which suffer from scalability issues \cite{unar2014review}. \ignore{With an increasing reliance on protected devices, a user can be overwhelmed with passwords or PIN requests to obtain access to various data and services. Knowledge-based approaches also require user interactions with the display, which may either be inconvenient to certain class of users or even completely absent in many wearables~\cite{unar2014review,zeng2017wearia}.}Many times, users opt to completely disable security mechanisms out of convenience, as the design hinders the implementation of security itself.



\subsection{Related Work}

\subsubsection{Wearable Constraints}
Wearable device user authentication is a relatively new field of research compared to other mobile authentication~\cite{bianchi2016wearable,blasco2016survey,cornelius2012wears,unar2014review}.
The limited display sizes of wearables add another constraint that limits the choices of authentication mechanisms~\cite{bianchi2016wearable,vhaduri2017wearable}. But as technology advances companies such as Samsung, Fit-bit, Apple, Garmin, and Embrace can provide low level granularity in data. In addition to this increasingly more biometrics are available as more sensors are being added such as microphone, electrocardiograms (ECG), and GPS. However still some limitations such as reading from ECG for example are not yet up to medical standards. Researchers have found that, although for people over the age of 85 Apple accurately detects atrial fibrillation at a rate of 96\%, for people under 55 it only correctly diagnoses atrial fibrillation 19.6\% of the time~\cite{Apple_ECG}. However, given better ECG technology, implicit authentication models will have a better performance. Another group of researchers~\cite{yan2019towards} developed designed wrist strapped ECG reader and developed an authentication system with an accuracy of 93.5\%, which is limited by the ease of use and placement issues. Therefore, an authentication scheme that can utilize data from readily available sensors on market wearables, such as the photo-plethysmography (PPG), accelerometer, gyroscope, and microphone, could be more realistic to develop a non-stop implicit wearable device user authentication system. 

\subsubsection{Multi-modal Biometric Authentication}
In previous work, combinations of biometrics were used to form multi-modal biometric authentication systems for increased reliability compared to unimodal systems, which often suffer from noisy data, intra-class variations, inter-class similarities, and spoof attacks~\cite{ghayoumi2015review}. For multi-modal authentication systems, researchers have utilized different hard- and soft-biometrics. However, due to accuracy concerns in sensing capabilities and relatively low computational power of wearables, these multi-modal approaches are typically not implemented for implicit and continuous authentication on state-of-the-art wearables. 


\subsubsection{Wearable Authentication}
 Researchers recently proposed authentication techniques that are more suitable for wearables, focusing more on approaches based on {\em behavioral biometrics}, such as gait~\cite{al2017unobtrusive,cola2016gait,johnston2015smartwatch}, activity types~\cite{bianchi2016wearable,zeng2017wearia}, gesture~\cite{davidson2016smartwatch}, keystroke dynamics~\cite{acar2018waca} and {\em physiological biometrics}, such as PPG signals~\cite{karimian2017non}. Almost all of these studies are based on project specific generated datasets\ignore{ databases and the accuracy of these techniques is often verified with limited numbers of subjects and over short time periods}. All of these user authentication techniques are limited in the scope of use, e.g., gait-based behavioral authentication approaches~\cite{cola2016gait,johnston2015smartwatch} only work during walking. While other projects have addressed some of the limitations of gait-based approaches by considering different types of gestures~\cite{davidson2016smartwatch} or activities~\cite{bianchi2016wearable,zeng2017wearia}. All of these models are based on movement and thereby, fail to work in the very common human state of being sedentary~\cite{acar2018waca,vhaduri2017wearable}. Authentication approaches using physiological biometric data, such as heart rate and bioimpedance~\cite{cornelius2012wears} require very fine-grained samples and sensor readings are easily affected by noise, motion, etc but are constantly available. Focusing on one or a particular set of biometrics restricts the usability of a continuous authentication model, but with a collection of various combinations it is possible to build a more robust authentication process. This method should be able continue and adjust when certain biometrics become unavailable or available.


\subsection{Contributions}
The main contribution of this paper is an exploration of multi-biometric model implicit or non-stop user authentication. 
The model approach used three different types of soft-biometrics: heart rate, gait, and breathing; all of which are easily obtainable on most of the market wearables.
Compared to previous work~\cite{vhaduri2017wearable,vhaduri2019multi}, where we use hybrid-biometrics, such as calorie burn that can be affected by a user's self-reported input, such as age, height, and weight, in this work we focus on the different biometrics that can be measured without the user's self-reported input. 
While minute-level coarse-grained heart rate samples can be less informative, they are available almost all the time when a user wear the device. Adding another biometric, such as gait, can improve the performance. However, unlike the heart rate data, gait is available only when a user moves. Compared to gait, breathing audio signal can have a better availability, but it also suffers from various issues, such as a user's distance from the microphone, presence of other sounds. Therefore, it is important to develop a multi-biometric-based approach that can be easy to implement on wearables and can have a way to decide which modalities should be used based on contexts or scenarios. In this work, we present a multi-biometric-based context-driven approach that works both in {\em sedentary} and {\em non-sedentary} periods (Section~\ref{approach}). From our detailed feature computation and selection, hyper-parameter optimization, and finally, modeling with different classifiers, we are able to authenticate a user with an average accuracy of $0.94 \pm 0.07$, $F_1$ score $0.94 \pm 0.07$ (Section~\ref{model_performance}), with FPR and FNR of about $0.06$ at 52\% level of confidence while classifying in the binary approach. Considering the situation where we do not have other users's data, we develop unary models which allows for offline training since other users data do not need to be downloaded. The unary models show a average accuracy of $0.72 \pm 0.07$, $F_1$ score $0.73 \pm 0.06$ also discussed in Section~\ref{model_performance}
